A Coefficient Makes SVRG Effective

Stochastic Variance Reduced Gradient (SVRG), introduced by Johnson & Zhang (2013), is a theoretically compelling optimization method. However, as Defazio & Bottou (2019) highlight, its effectiveness in deep learning is yet to be proven. In this work, we demonstrate the potential of SVRG in optimizing real-world neural networks. Our empirical analysis finds that, for deeper neural networks, the strength of the variance reduction term in SVRG should be smaller and decrease as training progresses. Inspired by this, we introduce a multiplicative coefficient $\alpha$ to control the strength and adjust it through a linear decay schedule. We name our method $\alpha$-SVRG. Our results show $\alpha$-SVRG better optimizes models, consistently reducing training loss compared to the baseline and standard SVRG across various model architectures and multiple image classification datasets. We hope our findings encourage further exploration into variance reduction techniques in deep learning. Code is available at github.com/davidyyd/alpha-SVRG.

==> figures/optimal_svrg_other_datasets.tex <==
\begin{figure}[th]
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/baseline_vs_optimal_svrg_sgd_eurosat_var_0.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/baseline_vs_optimal_svrg_sgd_eurosat_var_1.pdf}
\end{minipage}
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/baseline_vs_optimal_svrg_sgd_eurosat_var_2.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/baseline_vs_optimal_svrg_sgd_eurosat_loss.pdf}
\end{minipage}
\vspace{-.5em}
\caption{\textbf{SVRG with optimal coefficient on MLP-4.} SVRG with the optimal coefficient reduces gradient variance stably and achieves a substantially lower training loss than the baseline SGD.}
\label{fig:optimal_svrg_other_datasets}
\end{figure}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/ablation1.tex <==
\begin{figure}[t]
\centering
\begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,keepaspectratio]{graphs/coefficient.pdf}
    \vspace*{-2em}
    \caption{\textbf{Coefficient value.} \approach\ is effective with a wide range of coefficient values.}
    \label{fig:coef}
\end{minipage}%
\hfill
\begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,keepaspectratio]{graphs/batch_size.pdf}
    \vspace*{-2em}
    \caption{\textbf{Batch size.} \approach's effectiveness is observed for larger batch sizes.}
    \label{fig:batch}
\end{minipage}
\end{figure}


==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/ablation2.tex <==
\begin{figure}[h]
\centering
    \centering
    \includegraphics[width=.48\textwidth,keepaspectratio]{graphs/snapshot.pdf}
    \vspace*{-.5em}
    \caption{\textbf{Inner loop size.} Although a greater inner loop size leads to a weakening correlation between the model gradients and the snapshot gradients, \approach\ can still lower training loss.}
    
    \label{fig:snapshot}
\end{figure}


==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/baseline_vs_0.5svrg_adam.tex <==
\begin{figure}[bh]
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_alpha_svrg_adamw_var_0.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_alpha_svrg_adamw_var_1.pdf}
\end{minipage}
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_alpha_svrg_adamw_var_2.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_alpha_svrg_adamw_loss.pdf}
\end{minipage}
\caption{\textbf{$\boldsymbol{\alpha}$-SVRG with AdamW on MLP-4}. \approach\ can lower the gradient variance at the first 10 epochs, leading to a faster convergence than the baseline AdamW.}
\label{fig:svrg_vs_0.5_svrg_adam}
\end{figure}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/baseline_vs_svrg1.tex <==
\begin{figure}[h]
\centering
\vspace{-.5em}
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_svrg_linear_var_0.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_svrg_linear_var_1.pdf}
\end{minipage}
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_svrg_linear_var_2.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_svrg_linear_sgd_loss.pdf}
\end{minipage}
\vspace{-.5em}
\caption{\textbf{SVRG on Logistic Regression.} SVRG effectively reduces the gradient variance for Logistic Regression, leading to a lower training loss than the baseline.}
\label{fig:baseline_vs_svrg_1}
\end{figure}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/baseline_vs_svrg4.tex <==
\begin{figure}[!bh]
\centering
\vspace{-.5em}
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_svrg_var_0.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_svrg_var_1.pdf}
\end{minipage}
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_svrg_var_2.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_svrg_sgd_loss.pdf}
\end{minipage}
\vspace{-.5em}
\caption{\textbf{SVRG on MLP-4.} In the first few epochs, SVRG reduces the gradient variance for MLP-4, but afterward, SVRG increases it, well above the baseline. As a result, SVRG exhibits a higher training loss than the baseline at the end of training.}
\label{fig:baseline_vs_svrg_4}
\vspace{-1em}
\end{figure}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/convnext.tex <==

\begin{figure}[h]
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/convnext_var_0.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/convnext_var_1.pdf}
\end{minipage}
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/convnext_var_2.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/convnext_loss.pdf}
\end{minipage}
\caption{\textbf{$\boldsymbol{\alpha}$-SVRG on ConvNeXt-Femto}. \approach\ can reduce the gradient variance for ConvNeXt-Femto during the first 10 epochs (zoom-in plot) without increasing it later on. Consequently, $\alpha$-SVRG can decrease the training loss at a faster rate than the baseline AdamW.}
\label{fig:convnext}
\end{figure}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/correlation.tex <==
\begin{figure}[h]
    \centering
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth,keepaspectratio]{graphs/std0.pdf}
        \vspace*{-0.7cm}
        \centering
        \caption*{\hspace{0.05\linewidth} (a) SGD}
    \end{minipage}~
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth,keepaspectratio]{graphs/std1.pdf}
        \vspace*{-0.7cm}
        \centering
        \caption*{\hspace{0.05\linewidth} (b) AdamW}
    \end{minipage}
    \vspace*{-0.1cm}
    \caption{\textbf{Standard deviation ratio.} The ratio between the standard deviations of the model gradients and the snapshot gradients oscillates around 1 but is relatively stable overall.}
    \label{fig:std}
    \end{figure}
    \begin{figure}[h]
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth,keepaspectratio]{graphs/corr0.pdf}
        \vspace*{-0.7cm}
        \centering
        \caption*{\hspace{0.05\linewidth} (a) SGD}
    \end{minipage}~
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth,keepaspectratio]{graphs/corr1.pdf}
        \vspace*{-0.7cm}
        \centering
        \caption*{\hspace{0.05\linewidth} (b) AdamW}
    \end{minipage}
    \caption{\textbf{Correlation.} The correlation between the snapshot gradients and the model gradients decreases as the training progresses.}
    \label{fig:corr}
\end{figure}



==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/depth.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth,keepaspectratio]{graphs/optimal_coefficient0.pdf}
        \vspace*{-0.7cm}
        \centering
        \caption*{\hspace{0.05\linewidth} (a) SGD}
    \end{minipage}~
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth,keepaspectratio]{graphs/optimal_coefficient1.pdf}
        \vspace*{-0.7cm}
        \centering
        \caption*{\hspace{0.05\linewidth} (b) AdamW}
    \end{minipage}
    \caption{\textbf{Optimal coefficient.} At the start of each epoch, a snapshot is taken. Consequently, the optimal coefficient initiates at a value of 1 and results in a periodic upward jump.}
    \label{fig:depth}
\end{figure}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/optimal_coefficient_with_data.tex <==
\begin{figure}[h]
    \centering
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth,keepaspectratio]{graphs/optimal_coefficient_cifar10.pdf}
        \vspace*{-0.7cm}
        \centering
        \caption*{\hspace{0.05\linewidth} (a) CIFAR-10}
    \end{minipage}~
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth,keepaspectratio]{graphs/optimal_coefficient_cifar100.pdf}
        \vspace*{-0.7cm}
        \centering
        \caption*{\hspace{0.05\linewidth} (b) CIFAR-100}
    \end{minipage}
    \vspace*{-0.1cm}
    \caption{\textbf{Effects of Data on Optimal Coefficient.}}
    \vspace*{-0.1cm}
    \label{fig:optimal_data}
\end{figure}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/optimal_svrg_other_datasets.tex <==
\begin{figure}[th]
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/baseline_vs_optimal_svrg_sgd_eurosat_var_0.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/baseline_vs_optimal_svrg_sgd_eurosat_var_1.pdf}
\end{minipage}
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/baseline_vs_optimal_svrg_sgd_eurosat_var_2.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/baseline_vs_optimal_svrg_sgd_eurosat_loss.pdf}
\end{minipage}
\vspace{-.5em}
\caption{\textbf{SVRG with optimal coefficient on MLP-4.} SVRG with the optimal coefficient reduces gradient variance stably and achieves a substantially lower training loss than the baseline SGD.}
\label{fig:optimal_svrg_other_datasets}
\end{figure}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/optimal_svrg_vs_0.5svrg.tex <==
\begin{figure}[h]
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/optimal_svrg_vs_alpha_svrg_sgd_var_0.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/optimal_svrg_vs_alpha_svrg_sgd_var_1.pdf}
\end{minipage}
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/optimal_svrg_vs_alpha_svrg_sgd_var_2.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/optimal_svrg_vs_alpha_svrg_sgd_loss.pdf}
\end{minipage}
\caption{\textbf{$\boldsymbol{\alpha}$-SVRG on MLP-4.} \approach\ behaves similarly to SVRG with optimal coefficient.}
\label{fig:optimal_svrg_vs_0.5svrg}
\end{figure}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/schedule.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth,keepaspectratio]{graphs/schedule.pdf}
        \centering
        \vspace{-1.5em}
        \caption{global schedules}
        \label{fig:global_schedules}
    \end{subfigure}%
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth,keepaspectratio]{graphs/double_schedule.pdf}
        \centering
        \vspace{-1.5em}
        \caption{double schedules}
        \label{fig:double_schedules}
    \end{subfigure}
    \vspace*{-0.1cm}
    \caption{\textbf{Different coefficient schedules with $\boldsymbol{\alpha_0=0.75}$.} Each global schedule (left) maintains a static coefficient within an epoch and applies a coefficient decay only at the end of each epoch. In contrast, each double schedule (right) also adjusts the coefficient within an epoch.}
    \label{fig:schedule}
\end{figure*}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/svrg_vs_optimal_svrg.tex <==
\begin{figure}[th]
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_optimal_svrg_sgd_var_0.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_optimal_svrg_sgd_var_1.pdf}
\end{minipage}
\centering
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_optimal_svrg_sgd_var_2.pdf}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{graphs/variance_seed_pdf/baseline_vs_optimal_svrg_sgd_loss.pdf}
\end{minipage}
\caption{\textbf{SVRG with optimal coefficient on MLP-4.} SVRG with the optimal coefficient reduces gradient variance stably and achieves a lower training loss than the baseline SGD.}
\label{fig:svrg_vs_optimal_svrg}
\end{figure}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/figures/teaser.tex <==
\begin{figure}[h]
\vspace{-1.5em}
    \centering
    \begin{tikzpicture}
\node[above right] (img) at (0,0) {\includegraphics[width=\linewidth, keepaspectratio]{graphs/teaser.pdf}};
\node at (304pt,89pt) {$\alpha$};
\end{tikzpicture}
\vspace{-2em}
\caption{\textbf{SVRG vs. \(\boldsymbol{\alpha}\)-SVRG.}  Both SVRG (left) and \approach\ (right) use the difference between snapshot stochastic gradient (\textcolor{gray2}{gray}) and snapshot full gradient (\textcolor{blue}{blue}) to form a variance reduction term (\textcolor{orange}{orange}), which modifies model stochastic gradient (black) into variance reduced gradient (\textcolor{red2}{red}). But \approach\ employs a coefficient \(\alpha\) to modulate the strength of the variance reduction term. With this coefficient, \approach\ reduces the gradient variance and results in faster convergence.}
\label{fig:teaser}
\end{figure}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/sections/abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
   Stochastic Variance Reduced Gradient (SVRG), introduced by~\citet{johnson2013accelerating}, is a theoretically compelling optimization method. However, as~\cite{defazio2019ineffectiveness} highlight, its effectiveness in deep learning is yet to be proven. In this work, we demonstrate the potential of SVRG in optimizing real-world neural networks. Our empirical analysis finds that, for deeper neural networks, the strength of the variance reduction term in SVRG should be smaller and decrease as training progresses. Inspired by this, we introduce a multiplicative coefficient $\alpha$ to control the strength and adjust it through a linear decay schedule. We name our method \approach. Our results show \approach\ better optimizes models, consistently reducing training loss compared to the baseline and standard SVRG across various model architectures and multiple image classification datasets. We hope our findings encourage further exploration into variance reduction techniques in deep learning. Code is available at \url{github.com/davidyyd/alpha-SVRG}.
\end{abstract}


==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/sections/conclusion.tex <==
\section{Conclusion}
Over the past decade, SVRG has been a method with a significant impact on the theory of optimization. In this work, we explore the effectiveness of SVRG in training real-world neural networks. Our key insight is the optimal strength for the variance reduction term in SVRG is not necessarily 1. It should be lower for deeper networks and decrease as training advances. This motivates us to introduce \approach: applying a linearly decreasing coefficient $\alpha$ to SVRG. \approach\ leads to a steady reduction in gradient variance and optimizes models better. Our experiments show that \approach\ consistently achieves a lower training loss compared to both baseline and the standard SVRG. Our results motivate further research of variance reduction methods in neural networks training.

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/sections/experiments.tex <==
\section{Experiments}
\label{sec:experi}
\subsection{Settings}
\textbf{Datasets.} We evaluate \approach\ using ImageNet-1K classification~\citep{ImageNet1k} as well as smaller image classification datasets: CIFAR-100~\citep{cifar}, Pets~\citep{pets}, Flowers~\citep{flowers}, STL-10~\citep{stl10}, Food-101~\citep{food101}, DTD~\citep{dtd}, SVHN~\citep{svhn}, and EuroSAT~\citep{eurosat1}.

\textbf{Models.}
We use recently proposed vision models on ImageNet-1K, categorized into two groups: (1) smaller models with 5-19M parameters, including ConvNeXt-F~\citep{convnext-f, convnextzhuang}, ViT-T/16~\citep{vit}, Swin-F~\citep{swin}, and Mixer-S/32~\citep{mlp-mixer}; (2) larger models featuring 86M and 89M parameters: ViT-B/16 and ConvNeXt-B. ConvNeXt-F is also evaluated on all smaller image classification datasets.

\textbf{Training.}
We report both final epoch training loss and top-1 validation accuracy. Our basic training setting follows ConvNeXt~\citep{convnextzhuang}, which uses AdamW. Both SVRG and $\alpha$-SVRG also use AdamW as the base optimizer.  On small datasets, we choose the best $\alpha_0$ from \{0.5, 0.75, 1\}. We find the coefficient is robust and does not require extensive tuning. Therefore, for ImageNet-1K, we set $\alpha_0$ to 0.75 for smaller models and 0.5 for larger ones. Other training settings for \approach\ remain the same as the baseline. Further experimental settings can be found in Appendix \ref{appendix:setting}. 

\input{tables/pre-trained1}
\input{tables/pre-trained2}
\subsection{Results}
Table~\ref{tab:pre-trained1} presents the results of training various models on ImageNet-1K. The standard SVRG often increases the training loss, especially for larger models. In contrast, \approach\ decreases the training loss for both smaller and larger models. This also supports our earlier finding that deeper models benefit from lower coefficient values, and using a default coefficient of 1 impedes convergence.

Table~\ref{tab:pre-trained2} displays the results of training ConvNeXt-F on various smaller datasets. The standard SVRG generally elevates the training loss and impairs the generalization. On the contrary, \approach\ lowers the training loss and improves the validation accuracy across all small datasets. We have provided additional experiment results to demonstrate $\alpha$-SVRG's effectiveness in Appendix~\ref{appendix:additional_experiments}. 

Note that a lower training loss in \approach\ does not always lead to better generalization. For smaller models, a lower training loss usually directly translates to a higher validation accuracy. In larger models (Mixer-S, ViT-B, and ConvNeXt-B), additional adjustments to regularization strength may be needed for better generalization. This is out of scope for \approach\ as an optimization method but warrants future research on co-adapting optimization and regularization. 

\subsection{Analysis}
\label{sec:analysis}
We analyze various components in \approach. In the following experiments, we use an initial value $\alpha_0=0.5$ and ConvNeXt-F on STL-10 as the default setting. Because the standard SVRG is ineffective as discussed above, we omit it and only compare \approach\ to an AdamW baseline.

\textbf{Coefficient value.} We investigate the impact of the initial value of the coefficient \(\alpha_0\) for \approach. We vary it between 0 and 1 and observe its effect on the training loss. The results are presented in Figure~\ref{fig:coef}. The favorable range for initial values in \approach\ is quite broad, ranging from 0.2 to 0.9. This robustness indicates \approach\ requires minimal tuning in the practical setting. 

\input{figures/ablation1}
\textbf{Batch size.} Since the batch size controls the variance among mini-batch data, we change the batch size to understand how it affects \approach. We also scale the learning rate linearly~\citep{Goyal2017}. The default batch size is 128. In Figure~\ref{fig:batch}, we can see that \approach\ leads to a lower training loss when the batch size is larger, but it is worse than the baseline when the batch size is smaller. This may stem from the weakening correlation between snapshot gradients and model gradients as the batch size decreases. Therefore, a sufficiently large batch size is essential for \approach.


\textbf{Coefficient schedule.} By default, our $\alpha$-SVRG uses a linearly decreasing schedule to adjust the coefficient. Below we explore other schedules and illustrate them in Figure~\ref{fig:schedule}. Global schedules only decay the coefficient \emph{across epochs and keep as a constant within an epoch}. In contrast, double schedules also model the local decay in each epoch (Figure~\ref{fig:depth}) by initiating the coefficient at 1 and decreasing to an ending value specified by the global decay. More details on them are in Appendix~\ref{appendix:schedule}.

\input{figures/schedule}

Table~\ref{tab:schedule} presents the results of {\approach} using each schedule. \approach\ with double schedules surprisingly have a higher training loss than the AdamW baseline (1.64). This is possibly because the coefficient within an epoch sometimes overestimates the optimal coefficient and therefore increases gradient variance. In contrast, \approach\ with global schedules consistently achieves a lower training loss than the baseline (1.64) regardless of the choice of any initial coefficient.  

\input{tables/schedule}

\input{figures/ablation2}
\textbf{Inner loop size.} The inner loop size specifies the number of iterations between two consecutive snapshot captures. We vary it from 1 to 312 iterations to understand its effect on \approach. The default value is 39 iterations (one epoch). Figure~\ref{fig:snapshot} illustrates \approach\ has a lower training loss than the baseline even with a larger inner loop size, where the snapshot is relatively distant from the current model. On the other hand, a smaller inner loop size results in a lower training loss but requires additional training time, as a full gradient must be calculated each time a snapshot is taken.


==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/sections/introduction.tex <==
\section{Introduction}
A decade ago,~\citet{johnson2013accelerating} proposed a simple approach for reducing gradient variance in SGD---Stochastic Variance Reduced Gradient (SVRG). SVRG keeps a snapshot model and uses it to form a variance reduction term to adjust the gradient of the current model. This variance reduction term is the difference between the snapshot's stochastic gradient and its full gradient on the whole dataset. Utilizing this term, SVRG can reduce gradient variance of SGD and accelerate it to almost as fast as the full-batch gradient descent in strongly convex settings. 

Over the years, numerous SVRG variants have emerged. Some focus on further accelerating convergence in convex settings~\citep{xiao2014proximal, lin2015universal, defazio2016simple}, while others are tailored for non-convex scenarios~\citep{allenzhu2016variance, reddi2016stochastic, lei2017nonconvex, fang2018spider}. SVRG and its variants have shown effectiveness in optimizing simple machine learning models like logistic regression and ridge regression~\citep{allenzhu2018katyusha, lei2017nonconvex}.

Despite the theoretical value of SVRG and its subsequent works, they have seen limited practical success in training neural networks. Most SVRG research in non-convex settings is restricted to modest experiments: training basic models like Multi-Layer Perceptrons (MLP) or simple CNNs on small datasets like MNIST and CIFAR-10. These studies usually exclude evaluations on more capable and deeper networks. More recently,~\citet{defazio2019ineffectiveness} have exploited several variance reduction methods, including SVRG, to deep vision models. They found that SVRG fails to reduce gradient variance for deep neural networks because the model updates so quickly on the loss surface that the snapshot model becomes outdated and ineffective at variance reduction.

\input{figures/teaser}
In this work, we show that adding a multiplicative coefficient to SVRG's variance reduction term can make it effective for deep neural networks. Our exploration is motivated by an intriguing observation: SVRG can only reduce gradient variance in the initial training stages but \emph{increases} it later. To tackle this problem, we mathematically derive the optimal coefficient for the variance reduction term to minimize the gradient variance. Our empirical analysis then leads to two key observations about this optimal coefficient: (1) as the depth of the model increases, the optimal coefficient becomes smaller; (2) as training advances, the optimal coefficient decreases, dropping well below the default coefficient of 1 in SVRG. These findings help explain why a constant coefficient of 1 in SVRG, while initially effective, eventually fails to reduce gradient variance.

Based on these observations, we introduce a linearly decaying coefficient $\alpha$ to control the strength of the variance reduction term in SVRG. We call our method \approach\ and illustrate it in Figure~\ref{fig:teaser}. \approach\ decreases gradient variance stably across both early and late training and helps optimize the model better.  We evaluate \approach\ on a range of architectures and image classification datasets. \approach\ achieves a lower training loss than the baseline and the standard SVRG. Our results highlight the value of SVRG in deep learning. We hope our work can offer insights about SVRG and stimulate more research in variance reduction approaches for optimization in neural networks.


==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/sections/method.tex <==
\section{Motivation: SVRG may not always reduce variance}
\label{sec:motivation}
\textbf{SVRG formulation.} We first introduce the basic formulation of SVRG. We adopt the following notation: \(t\) is the iteration index, \(\vtheta^t\) represents the current model parameters, and \(\nabla f_i(\cdot)\) denotes the gradient of loss function $f$ for the $i$-th mini-batch. In SVRG's original work~\citep{johnson2013accelerating}, this corresponds to the $i$-th data point. When the subscript $i$ is omitted, \(\nabla f(\cdot)\) represents the full gradient across the entire dataset. A key concept in SVRG is the snapshot model, represented as \(\snapshot\). It is a snapshot of the model at a previous iteration before $t$. We store its full gradient \(\nabla f(\snapshot)\). This snapshot is taken periodically. SVRG defines the variance reduced gradient \(\vg_i^t\), as follows:
\begin{gather}
    \vg_i^t = \nabla f_i(\vtheta^t)-\underbrace{(\nabla f_i(\snapshot)-\nabla f(\snapshot))}_\text{variance reduction term}\label{eq:svrg}.
\end{gather}
Intuitively, SVRG uses the difference between the mini-batch gradient and full gradient of a past model to modify the current mini-batch gradient. This could make \(\vg_i^t\) better aligned with the current full gradient $\nabla f(\vtheta^t)$ and thus stabilize each update.

SVRG was initially introduced in the context of vanilla SGD. Recent work~\citep{adasvrg,adamsvrg} has integrated SVRG into alternative base optimizers. Following them, we input the variance reduced gradient \(\vg_i^t\) into the base optimizer and ensure a fair comparison by using the same base optimizer for SVRG and the baseline. We also follow the practice in~\cite{defazio2019ineffectiveness}, taking snapshot for SVRG once per training epoch.


\input{tables/metric}
\textbf{Gradient variance.} Our goal is to assess SVRG's effectiveness in reducing gradient variance. To this end, we gather $N$ mini-batch gradients, denoted as \(\{\vg_i^t|i\in\{1,\cdots,N\}\}\), by performing back-propagation on checkpoints of the model at the iteration \(t\) with randomly selected $N$ mini-batches. For SVRG, each of these gradients is modified based on Equation~\ref{eq:svrg}. To present a comprehensive view, we employ three metrics from prior studies to quantify gradient variance in Table~\ref{tab:metric}.

In this part, we compare our three metrics. Metric 1 calculates the cosine distance between pairwise mini-batch gradients, therefore only capturing variance in gradient directions rather than gradient magnitudes. This is very important for scale-invariant optimizers, such as Adagrad~\citep{adagrad} and Adam~\citep{adam}. In contrast, metric 2 focuses on both gradient directions and magnitudes by summing the variance of each component of gradients. This metric has been the standard tool to measure gradient variance in various optimization literature~\citep{allenzhu2016variance, defazio2019ineffectiveness}. Metric 3 considers the largest eigenvalue in gradient covariance matrix, characterizing the most dominant part in gradient variance. We also average each gradient variance metric across three runs, with shaded regions in figures representing the standard deviation.

\textbf{SVRG's effect on gradient variance.} To understand how SVRG affects training, we examine two simple models: a linear layer (Logistic Regression) and a 4-layer Multi-Layer Perceptron (MLP-4). We train them over 30 epochs on CIFAR-10. We compare SVRG to a baseline using only SGD.

\input{figures/baseline_vs_svrg1}

We plot Logistic Regression's gradient variance (top two and bottom left) and training loss (bottom right) in Figure~\ref{fig:baseline_vs_svrg_1}. For Logistic Regression, SVRG can reduce the gradient variance throughout the entire training process and achieve a lower training loss than the baseline.

\input{figures/baseline_vs_svrg4}
In contrast, for MLP-4, SVRG may not always reduce gradient variance. As shown in Figure~\ref{fig:baseline_vs_svrg_4}, SVRG can only decrease the gradient variance for the first five epochs but then increases it. Consequently, SVRG has a larger final training loss than the baseline. This indicates that the increase in gradient variance caused by SVRG hinders the convergence of MLP-4's training loss.

This surprising empirical observation in a slightly deeper model leads us to question whether SVRG may alter the gradient too excessively at certain phases of training. Can we mitigate this adverse effect? We explore these questions starting from a theoretical framework in the next section.

\section{A Closer Look at Control Variates in SVRG}
\label{sec:3}
Control variates~\citep{lavenberg1977application} is a technique initially developed in Monte Carlo methods to reduce variance. We aim to estimate the expected value of a random variable \(\ermX\). The variance of this estimate usually depends on \(\Var(\ermX)\). To form a less variate estimate \(\ermX^*\), we can use a control variate \( \ermY \) that correlates with \(\ermX \) and a coefficient \( \alpha \) to regulate the influence of \( \ermY \) and \( \mathbb{E}[\ermY] \) :
\begin{gather}
    \ermX^* = \ermX - \alpha (\ermY - \mathbb{E}[\ermY]).\label{eq:control}
\end{gather}
This estimate remains unbiased for any value of \( \alpha \). The coefficient that minimizes the variance of the estimate can be derived as:
\begin{gather}
\alpha^* = \frac{\Cov(\ermX, \ermY)}{\Var(\ermY)}=\rho(\ermX, \ermY)\frac{\sigma(\ermX)}{\sigma(\ermY)},\label{eq:control_opt}
\end{gather}
where \(\rho(\ermX,\ermY)\) represents the correlation coefficient between \(\ermX\) and \(\ermY\); \(\sigma(\cdot)\) denotes the standard deviation. The derivation is detailed in Appendix~\ref{appendix:derivation}. 
The minimized variance becomes \(\Var(\ermX^*) = (1-\rho(\ermX,\ermY)^2)\Var(\ermX)\). The higher the correlation is, the lower the variance of the estimate is.

Note that SVRG uses control variates to reduce variance in each component of the gradient. This variance reduction occurs at each iteration \(t\). Take a closer look at Equation~\ref{eq:svrg} and~\ref{eq:control}: the model stochastic gradient \(f_i(\vtheta^t)\) is the random variable \(\ermX\); the snapshot stochastic gradient \(f_i(\snapshot)\) is the control variate \(\ermY\); and the snapshot full gradient \(f(\snapshot)\) is the expectation \( \mathbb{E}[\ermY] \). 

A key difference between SVRG and control variates is that SVRG omits the coefficient \(\alpha\), defaulting it to 1. This is possibly because the gradient distribution does not change drastically in strongly convex settings~\citep{johnson2013accelerating}. Yet, SVRG's subsequent studies, even those addressing non-convex cases, have neglected the coefficient and formulated their theories based on Equation~\ref{eq:svrg}. 

Motivated by this, we introduce a time-dependent coefficient vector \( \boldsymbol{\alpha}^t \in \mathbb{R}^d \) in SVRG:
\begin{gather}
    \vg_i^t = \nabla f_i(\vtheta^t)-\boldsymbol{\alpha}^t\odot(\nabla f_i(\snapshot)-\nabla f(\snapshot)),\label{eq:approach}
\end{gather}
where \( \odot \) represents the element-wise multiplication.

\textbf{Optimal coefficient.}
We adopt the same gradient variance definition as~\citet{defazio2019ineffectiveness} (metric 2 in Table~\ref{tab:metric}) and aim to determine the optimal $\boldsymbol{\alpha}^{t*}$ that minimizes it at each iteration. Specifically, our objective is to minimize the sum of variances across each component of \( \vg_i^t \). Let $k$ index the $k$-th component \( \alpha^{t*}_k \) and the $k$-th component of the gradient \(\nabla f_{\cdot, k}(\cdot)\). For clarity, we omit the mini-batch index $i$. This can be formally expressed as follows:
\begin{gather}
    \min_{\boldsymbol{\alpha}^t} \sum_{k=1}^d \Var(g^t_{\cdot, k})=\sum_{k=1}^d \min_{\alpha^t_k} \Var(g^t_{\cdot, k}).\label{eq:switch}
\end{gather}
We can switch the order of minimization and summation in Equation~\ref{eq:switch} because the variance of the $k$-th component of the gradient only depends on the $k$-th component of the coefficient. Applying Equation~\ref{eq:control_opt} yields the optimal coefficient \(\alpha^{t*}_k\):
\begin{gather}
    \alpha^{t*}_k = \frac{\Cov(\nabla f_{\cdot,k}(\snapshot), \nabla f_{\cdot,k}(\vtheta^t))}{\Var(\nabla f_{\cdot,k}(\snapshot))} = \rho(\nabla f_{\cdot, k}(\snapshot), \nabla f_{\cdot, k}(\vtheta^t))\frac{\sigma(\nabla f_{\cdot, k}(\vtheta^t))}{\sigma(\nabla f_{\cdot, k}(\snapshot))}.\label{eq:optimal}
\end{gather}
A stronger correlation between the snapshot and model gradients leads to a larger optimal coefficient. 

For small networks like MLP-4, calculating the optimal coefficient at each iteration is feasible by gathering all mini-batch gradients for both the current and snapshot models. For larger networks, however, this method becomes impractical; we will address this challenge later in the paper.

\textbf{Observations on optimal coefficient.}
To explore how the optimal coefficient evolves in a normal training setting, we train 1, 2, and 4-layer MLPs (Logistic Regression, MLP-2, and MLP-4) using SGD and AdamW~\citep{adamw} on CIFAR-10 \textit{without using SVRG}. Given the small size of these models, we can analytically compute the optimal coefficient at each iteration. We plot its mean value over all indices $k$ in Figure~\ref{fig:depth}. 
 We can make two notable observations as below.

\input{figures/depth}
\emph{Observation 1: a deeper model has a smaller optimal coefficient.} For Logistic Regression, the optimal coefficient remains relatively stable, hovering near 1. For MLP-2, the coefficient deviates from 1, dropping to about 0.6. For MLP-4, it decreases more sharply, reaching approximately 0.4.

\emph{Observation 2: the average optimal coefficient of a deeper model in each epoch generally decreases as training progresses.} This suggests that each epoch's average correlation between snapshot gradients and model gradients ($\rho(\nabla f_{\cdot, k}(\snapshot), \nabla f_{\cdot, k}(\vtheta^t))$ in Equation~\ref{eq:optimal}) decreases as the model becomes better trained. We further analyze this decreasing trend of the correlation term in Appendix~\ref{appendix:corr}.

These observations shed light on why the standard SVRG struggles to reduce gradient variance or training loss in later training stages (Figure~\ref{fig:baseline_vs_svrg_4}). A default coefficient of 1 proves to be too high, and the weakening correlation between snapshot and model gradients necessitates a smaller coefficient. Without a suitable coefficient, gradient variance may increase, leading to oscillations in SGD.

\textbf{Optimal coefficient's effect on gradient variance.} We evaluate whether optimal coefficient can make SVRG more effective in reducing gradient variance. Specifically, we use SVRG with optimal coefficient to train an MLP-4 by computing optimal coefficient (Equation~\ref{eq:optimal}) and adjusting the gradient (Equation~\ref{eq:approach}) at each iteration. In Figure~\ref{fig:svrg_vs_optimal_svrg}, we compare SVRG with optimal coefficient to an SGD baseline. Using the optimal coefficient enables SVRG to reduce gradient variance in the early stages of training without uplifting it later. This yields a consistently lower training loss than the baseline.
\input{figures/svrg_vs_optimal_svrg}

\section{\approach}
\label{sec:approach}
From our analysis above, it becomes clear that the best coefficient for SVRG is not necessarily 1 for deep neural networks. However, computing the optimal coefficient at each iteration would result in a complexity of full-batch gradient descent. This approach quickly becomes impractical for larger networks like ResNet~\citep{He2016}. In this section, we show how using a preset schedule of $\alpha$ values can achieve a similar effect of using the computed optimal coefficients.

\textbf{\(\boldsymbol{\alpha}\)-SVRG.}  Given the decreasing trend (Figure~\ref{fig:depth}) and the computational challenge, we propose to apply a linearly decreasing scalar coefficient for SVRG, starting from an initial value $\alpha_0$ and decreasing to 0. This is our main method in this paper. We name it \approach. More results of enabling {\approach} only during the early stage of training are in Appendix~\ref{appendix:early_svrg}. The pseudocode for \approach\ with SGD and AdamW as base optimizers is provided in Appendix~\ref{appendix:pseudocode}.

\input{figures/optimal_svrg_vs_0.5svrg}
To evaluate how well {\approach} matches SVRG with optimal coefficient, we train an MLP-4 using {\approach} and compare it to SVRG with optimal coefficient. For all experiments in this section, we set \(\alpha_0=0.5\). The results are presented in Figure~\ref{fig:optimal_svrg_vs_0.5svrg}. Interestingly, {\approach} exhibits a gradient variance trend that is not much different from SVRG with optimal coefficient. Similarly, the training loss of {\approach} is only marginally larger than that of SVRG with optimal coefficient.  

\input{figures/baseline_vs_0.5svrg_adam} 

\textbf{\(\boldsymbol{\alpha}\)-SVRG with AdamW.} Since AdamW~\citep{adamw} is a widely used optimizer in modern neural network training, we assess the performance of {\approach} with AdamW. We change the base optimizer in {\approach} to AdamW and use it to train an MLP-4 on CIFAR-10. We compare {\approach} to a baseline using only AdamW. As shown in Figure~\ref{fig:svrg_vs_0.5_svrg_adam}, {\approach} has a noticeable gradient variance reduction initially and achieves a consistent lower training loss for MLP-4 than the baseline.

\textbf{\(\boldsymbol{\alpha}\)-SVRG on deeper networks.}
We further study the effectiveness of {\approach} with AdamW on real-world neural architectures, moving beyond simple MLPs. To this end, we train a modern ConvNet architecture, ConvNeXt-Femto~\citep{convnextzhuang,convnext-f}, on CIFAR-10 using the default AdamW optimizer. We compare {\approach} to the baseline using vanilla AdamW in Figure~\ref{fig:convnext}. {\approach} can reduce gradient variance during the first 10 epochs (zoom-in plot of Figure~\ref{fig:convnext}) and then maintain it at the same level as the baseline. As a result, the training loss of {\approach} converges much faster than the baseline. This demonstrates the potential of {\approach} in optimizing more complex models. We further explore this with additional experiments next.
\input{figures/convnext}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/sections/related_work.tex <==
\section{Related Work}
\textbf{Variance reduction in optimization.} There are a range of methods aiming at reducing gradient variance by directly modifying stochastic gradient. Initial works~\citep{johnson2013accelerating, sag} focus on simple convex settings. Subsequent research enhances these methods~\citep{defazio2014saga, miso, lin2015universal, defazio2016simple, allenzhu2018katyusha, lin2018catalyst} or handles finite sums in non-convex landscapes~\citep{allenzhu2016variance, nguyen2017sarah, fang2018spider, li2018simple, cutkosky2020momentumbasedvariancereductionnonconvex, elibol2020variance, zhou2020stochastic, adaspider}. For these methods, we either need to store all gradient with respect to each individual data point~\citep{sdca, defazio2014finito, li2021zerosarah} or calculate full gradient periodically~\citep{johnson2013accelerating, fang2018spider}. \citet{survey} provide a comprehensive review for variance reduction methods. While these studies focus on theories of SVRG, we primarily explore the practical utility of SVRG for real-world neural networks.

One of the most relevant works to us is MARS~\citep{yuan2024mars}, which also demonstrates that using a coefficient helps the variance reduction methods optimize modern neural networks. In contrast, our work studies how a coefficient makes SVRG effective through step-by-step controlled experiments.

\textbf{Implicit variance reduction.} Apart from methods that explicitly adjust the gradient, there are variance reduction techniques that implicitly reduce gradient variance through other means. A variety of optimizers~\citep{adadelta, adam, nadam, adagrad, adamw, radam, lion, sophia} utilize momentum to mitigate gradient variance. They achieve this by averaging past gradients exponentially, thus stabilizing subsequent updates. Lookahead optimizer~\citep{lookahead} reduces gradient variance by only updating the model once every $k$ iterations. Dropout~\citep{dropout1} is also found to reduce gradient variance and better optimize models when used at early training~\citep{liu2023dropout}.

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/tables/early.tex <==
\begin{table}[th]
\centering
\small
\def\arraystretch{1.3}
\begin{tabular}{lcccccccc}
& \multicolumn{2}{c}{CIFAR-100} & \multicolumn{2}{c}{Pets} & \multicolumn{2}{c}{Flowers} & \multicolumn{2}{c}{STL-10} \\
\Xhline{0.7pt}
AdamW & 2.659 & - & 2.203 & - & 2.400 & - & 1.641 & - \\
\rowcolor{gray} 
+\ \approach\ & 2.646 & \better{0.013} & 2.004 & \better{0.199} & 2.162 & \better{0.238} & 1.568 & \better{0.073} \\
\rowcolor{gray}
+\ early \approach\ & 2.644 & \better{0.015} & 2.190 & \better{0.013} & 2.328 & \better{0.072} & 1.616 & \better{0.025} \\
\end{tabular}

\centering
\small
\begin{tabular}{lcccccccccc}
& \multicolumn{2}{c}{Food-101} & \multicolumn{2}{c}{DTD} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{EuroSAT} \\
\Xhline{0.7pt}
AdamW & 2.451 & - & 1.980 & - & 1.588 & - & 1.247 & - \\
\rowcolor{gray}
+\ \approach\ & 2.461 & \worse{0.010} & 1.829 & \better{0.151} & 1.573 & \better{0.015} & 1.237 & \better{0.010} \\
\rowcolor{gray}
+\ early \approach\ & 2.444 & \better{0.007} & 1.918 & \better{0.062} & 1.583 & \better{0.005} & 1.240 & \better{0.007} \\
\end{tabular}
\caption*{(a) \textbf{training loss}}
\vspace{.5em}
\small
\begin{tabular}{lcccccccc}
& \multicolumn{2}{c}{CIFAR-100} & \multicolumn{2}{c}{Pets} & \multicolumn{2}{c}{Flowers} & \multicolumn{2}{c}{STL-10} \\
\Xhline{0.7pt}
baseline & 81.0 & - & 72.8 & - & 80.8 & - & 82.3 & - \\
\rowcolor{gray}
+\ \approach\ & 80.6 & \worseinv{0.4} & 76.7 & \betterinv{3.9} & 82.6 & \betterinv{1.8}  & 84.0 & \betterinv{1.7} \\
\rowcolor{gray}
+\ early \approach\ & 81.0 & \betterinv{0.0} & 74.6 & \betterinv{1.8} & 83.6 & \betterinv{2.8} & 82.8 & \betterinv{0.5}\\
\end{tabular}

\centering
\small
\begin{tabular}{lcccccccccc}
& \multicolumn{2}{c}{Food-101} & \multicolumn{2}{c}{DTD} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{Euro} \\
\Xhline{0.7pt}
baseline & 85.9 & - & 57.9 & - & 94.9 & - & 98.1 & - \\
\rowcolor{gray}
+\ \approach\ & 85.0 & \worseinv{0.9} & 60.3 & \betterinv{2.4} & 95.7 & \betterinv{0.8} & 98.2 & \betterinv{0.1} \\
\rowcolor{gray}
+\ early \approach\ & 85.9 & \betterinv{0.0} & 62.3 & \betterinv{4.4} & 95.8 & \betterinv{0.9} & 98.0 & \worseinv{0.1}\\
\end{tabular}
\caption*{(b) \textbf{validation accuracy}}
\caption{\textbf{Early $\boldsymbol{\alpha}$-SVRG on smaller classification datasets.} }
\label{tab:early}
\end{table}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/tables/hyper.tex <==
\begin{table}[bp]
    \centering
    \small
    \def\arraystretch{1.2}
    \addtolength{\tabcolsep}{-2.5pt}
    \begin{tabular}{lcccccccccc}
    &CIFAR-100 & Pets & Flowers & STL-10 & Food101 &DTD & SVHN & EuroSAT & ImageNet-1K \\
    \Xhline{0.7pt}
   batch size & 1024 & 128 & 128 & 128 & 1024 & 128 & 1024 & 512 & 4096\\
   warmup epochs & 50 & 100 & 100 & 50 & 50 & 100 & 20 & 40 & 50\\
   training epochs & 300 & 600 & 600 & 300 & 300 & 600 & 100 & 200 & 300
    \end{tabular}
    
    \caption{\textbf{Hyperparameter setting.}}
    \label{tab:hyper}
\end{table}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/tables/hyper2.tex <==
\begin{table}[th]
    \centering
    \small
    \def\arraystretch{1.2}
    \addtolength{\tabcolsep}{-1.4pt}
    \begin{tabular}{lcccccccccc}
    &CIFAR-100 & Pets & Flowers & STL-10 & Food101 &DTD & SVHN & EuroSAT \\
    \Xhline{0.7pt}
   batch size & 1024 & 128 & 128 & 128 & 1024 & 128 & 1024 & 512 \\
   training epochs & 150 & 200 & 150 & 200 & 50 & 200 & 50  & 100 
    \end{tabular}
    \caption{\textbf{Hyperparameter setting for {$\boldsymbol{\alpha}$-SVRG} with SGD on ResNet-18.}}
    \label{tab:hyper2}
\end{table}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/tables/metric.tex <==
\begin{table}[bp]
\centering
\small
\vspace{-.5em}
\begin{tabular}{c|cc}
name & formula & description\\
\Xhline{0.7pt}
metric 1* & $\frac{2}{N(N-1)}\sum_{i\neq j}\frac{1}{2}(1-\frac{\langle \vg_i^t,\vg_j^t\rangle}{\|\vg_i^t\|_2\|\vg_j^t\|_2})$& the directional variance of the gradients\\[3pt]
metric 2$\dagger$ & $\sum_{k=1}^d\Var(g_{i, k}^t)$& the variance of gradients across each component \\[4pt]
metric 3$\ddagger$ & $ \lambda_{max}(\frac{1}{N}\sum_{i=1}^N(\vg_i^t-\vg^t)(\vg_i^t-\vg^t)^T)$ & the magnitude of the most significant variation \\
\end{tabular}
\vspace{-.5em}
\caption{\textbf{Metrics.} $\vg^t$ is the mean of the mini-batch gradients $\vg_i^t$. $k$ indexes the $k$-th component of gradient $g_{i, k}^t$. References: $*$~\citet{liu2023dropout}, $\dagger$~\citet{defazio2019ineffectiveness}, $\ddagger$~\citet{jastrzebski2020breakeven}}
\label{tab:metric}
\end{table}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/tables/new.tex <==
\begin{table}[h]
\centering
\small
\def\arraystretch{1.3}
\vspace{-.5em}
\begin{tabular}{lcccccccc}
& \multicolumn{2}{c}{CIFAR-100} & \multicolumn{2}{c}{Pets} & \multicolumn{2}{c}{Flowers} & \multicolumn{2}{c}{STL-10} \\
\Xhline{0.7pt}
AdamW & 2.659 & - & 2.203 & - & 2.400 & - & 1.641 & - \\
+\ SVRG & 2.937 & \worse{0.278} & 3.424 & \worse{1.221} & 2.256 & \better{0.144} & 1.899 & \worse{0.258} \\
\rowcolor{gray}
+\ \approach\ $(\alpha_0=0.5)$ &  \textbf{2.622} & \better{0.037} & 1.960 & \better{0.243} & 2.265 & \better{0.135} & 1.583 & \better{0.058}\\
\rowcolor{gray}
+\ \approach\ $(\alpha_0=0.75)$ & 2.646 & \better{0.013} & 2.004 & \better{0.199} & \textbf{2.162} & \better{0.238} & \textbf{1.568} & \better{0.073} \\
\rowcolor{gray}
+\ \approach\ $(\alpha_0=1)$ & 2.712 & \worse{0.053} & \textbf{1.994} & \better{0.209} & 2.259 & \better{0.141} & 1.573 & \better{0.068} \\
\end{tabular}

\centering
\small
\begin{tabular}{lcccccccccc}
& \multicolumn{2}{c}{Food-101} & \multicolumn{2}{c}{DTD} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{EuroSAT} \\
\Xhline{0.7pt}
AdamW & 2.451 & - & 1.980 & - & 1.588 & - & 1.247 & - \\
+\ SVRG & 3.026 & \worse{0.575} & 2.009 & \worse{0.029} & 1.639 & \worse{0.051} & 1.249 & \worse{0.002} \\
\rowcolor{gray}
+\ \approach\ $(\alpha_0=0.5)$ & \textbf{2.423} & \better{0.028} & 1.865 & \better{0.115} & \textbf{1.572} & \better{0.016} & 1.243 & \better{0.004} \\
\rowcolor{gray}
+\ \approach\ $(\alpha_0=0.75)$ & 2.461 & \worse{0.010} & 1.829 & \better{0.151} & 1.573 & \better{0.015} & 1.237 & \better{0.010} \\
\rowcolor{gray}
+\ \approach\ $(\alpha_0=1)$ & 2.649 & \worse{0.198} & \textbf{1.790} & \better{0.190} & 1.585 & \better{0.003} & \textbf{1.230} & \better{0.017} \\
\end{tabular}
\caption*{(a) \textbf{training loss}}
\vspace{.5em}
\small
\begin{tabular}{lcccccccc}
& \multicolumn{2}{c}{CIFAR-100} & \multicolumn{2}{c}{Pets} & \multicolumn{2}{c}{Flowers} & \multicolumn{2}{c}{STL-10} \\
\Xhline{0.7pt}
AdamW & 81.0 & - & 72.8 & - & 80.8 & - & 82.3 & - \\
+\ SVRG & 78.2 & \worseinv{2.8} & 17.6 & \worseinv{55.2} &  82.6 & \betterinv{1.8} & 65.1 & \worseinv{17.2} \\
\rowcolor{gray}
+\ \approach\ $(\alpha_0=0.5)$ & \textbf{81.4} & \betterinv{0.4} & \textbf{77.8} & \betterinv{5.0} & \textbf{83.3} & \betterinv{2.5} & \textbf{83.5} & \betterinv{1.2} \\
\rowcolor{gray}
+\ \approach\ $(\alpha_0=0.75)$ & 80.6 & \worseinv{0.4} & 76.7 & \betterinv{3.9} & 82.6 & \betterinv{1.8}  & 84.0 & \betterinv{1.7} \\
\rowcolor{gray}
+\ \approach\ $(\alpha_0=1)$ & 80.0 & \worseinv{1.0} & 77.3 & \betterinv{4.5} & 81.9 & \betterinv{1.1} & 84.0 & \betterinv{1.7} \\
\end{tabular}

\centering
\small
\begin{tabular}{lcccccccccc}
& \multicolumn{2}{c}{Food-101} & \multicolumn{2}{c}{DTD} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{Euro} \\
\Xhline{0.7pt}
AdamW & \textbf{85.9} & - & 57.9 & - & 94.9 & - & 98.1 & - \\
+\ SVRG & 79.6 & \worseinv{6.3} & 57.8 & \worseinv{0.1} & 95.7 & \betterinv{0.8} & 97.9 & \worseinv{0.2} \\
\rowcolor{gray}
+\ \approach\ $(\alpha_0=0.5)$ & \textbf{85.9} & \betterinv{0.0} & 57.0 & \worseinv{0.9} & 95.4 & \betterinv{0.5} & \textbf{98.2} & \betterinv{0.1} \\
\rowcolor{gray}
+\ \approach\ $(\alpha_0=0.75)$& 85.0 & \worseinv{0.9} & 60.3 & \betterinv{2.4} & 95.7 & \betterinv{0.8} & \textbf{98.2} & \betterinv{0.1} \\
\rowcolor{gray}
+\ \approach\ $(\alpha_0=1)$ & 83.8 & \worseinv{2.1} & \textbf{61.8} & \betterinv{3.9} & \textbf{95.8} & \betterinv{0.9} & \textbf{98.2} & \betterinv{0.1} \\
\end{tabular}
\caption*{(b) \textbf{validation accuracy}}
\caption{\textbf{Results on smaller classification datasets with different initial coefficients.} While SVRG negatively affects performance on most of these datasets, \approach\ consistently reduces the training loss and improves the validation accuracy for almost any initial coefficient on each dataset.}
\label{tab:last}
\vspace{-.5em}
\end{table}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/tables/pre-trained1.tex <==
\begin{table}[t]
\def\arraystretch{1.3}
\addtolength{\tabcolsep}{-2pt}
\centering
\small
\begin{tabular}{lcccccccccccc}
& \multicolumn{2}{c}{ConvNeXt-F} & \multicolumn{2}{c}{ViT-T} & \multicolumn{2}{c}{Swin-F} & \multicolumn{2}{c}{Mixer-S} & \multicolumn{2}{c}{ViT-B} & \multicolumn{2}{c}{ConvNeXt-B} \\
\Xhline{0.7pt}
\multicolumn{13}{c}{training loss} \\
AdamW & 3.487 & - & 3.443 & - & 3.427 & - &  3.149 & - & 2.817 & - & 2.644 & - \\
+\ SVRG & 3.505 & \worse{.018} & 3.431 & \better{.012} & \textbf{3.389} & \better{.038} & 3.172 & \worse{.023} & 3.309 & \worse{.492} & 3.113 & \worse{.469} \\
\rowcolor{gray}
+\ \approach & \textbf{3.467} & \better{.020} & \textbf{3.415} & \better{.028} & 3.392 & \better{.035} & \textbf{3.097} & \better{.052} & \textbf{2.806} & \better{.011} & \textbf{2.642} & \better{.002} \\
\Xhline{0.7pt}
\multicolumn{13}{c}{validation accuracy} \\
AdamW & 76.0 & - & 73.9 & - & 74.3 & - & \textbf{76.4} & - & \textbf{81.6} & - & \textbf{83.7} & - \\
+\ SVRG & 75.7 & \worseinv{0.3} & \textbf{74.3} & \betterinv{0.4} & 74.3 & \betterinv{0.0} & 74.5 & \worseinv{1.9} & 78.0 & \worseinv{3.6} & 80.8 & \worseinv{2.9} \\
\rowcolor{gray}
+\ \approach & \textbf{76.3} & \betterinv{0.3} & 74.2 & \betterinv{0.3} & \textbf{74.8} & \betterinv{0.5} & 76.1 & \worseinv{0.3} & \textbf{81.6} & \betterinv{0.0} & 83.1 & \worseinv{0.6} \\
\end{tabular}
\caption{\textbf{Results on ImageNet-1K.} The standard SVRG increases the training loss for most models, whereas \approach\ consistently decreases it for all models.}
\label{tab:pre-trained1}
\end{table}


==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/tables/pre-trained2.tex <==
\begin{table}[ht]
\centering
\small
\addtolength{\tabcolsep}{-4.35pt}
\def\arraystretch{1.3}
\begin{tabular}{lcccccccccccccccc}
&\multicolumn{2}{c}{CIFAR-100} & \multicolumn{2}{c}{Pets} & \multicolumn{2}{c}{Flowers} & \multicolumn{2}{c}{STL-10} & \multicolumn{2}{c}{Food-101} & \multicolumn{2}{c}{DTD} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{EuroSAT} \\
\Xhline{0.7pt}

\multicolumn{17}{c}{training loss} \\
AdamW & 2.66 & - & 2.20 & - & 2.40 & - & 1.64 & - & 2.45 & - & 1.98 & - & 1.59 & - & 1.25 & - \\
+\ SVRG & 2.94 & \worse{0.28} & 3.42 & \worse{1.22} & 2.26 & \better{0.14} & 1.90 & \worse{0.26} & 3.03 & \worse{0.58} & 2.01 & \worse{0.03} & 1.64 & \worse{0.05} & 1.25 & 0.00 \\
\rowcolor{gray}
+\ \approach & \textbf{2.62} & \better{0.04} & \textbf{1.96} & \better{0.24} & \textbf{2.16} & \better{0.24} & \textbf{1.57} & \better{0.07} & \textbf{2.42} & \better{0.03} & \textbf{1.83} & \better{0.15} & \textbf{1.57} & \better{0.02} & \textbf{1.23} & \better{0.02} \\

\Xhline{0.7pt}
\multicolumn{17}{c}{validation accuracy} \\
AdamW & 81.0 & - & 72.8 & - & 80.8 & - & 82.3 & - & \textbf{85.9} & - & 57.9 & - & 94.9 & - & 98.1 & - \\
+\ SVRG & 78.2 & \worseinv{2.8} & 17.6 & \worseinv{55.2} &  82.6 & \betterinv{1.8} & 65.1 & \worseinv{17.2} & 79.6 & \worseinv{6.3} & 57.8 & \worseinv{0.1} & 95.7 & \betterinv{0.8} & 97.9 & \worseinv{0.2} \\
\rowcolor{gray}
+\ \approach & \textbf{81.4} & \betterinv{0.4} & \textbf{77.8} & \betterinv{5.0} & \textbf{83.3} & \betterinv{2.5} & \textbf{84.0} & \betterinv{1.7} & \textbf{85.9} & \betterinv{0.0} & \textbf{61.8} & \betterinv{3.9} & \textbf{95.8} & \betterinv{0.9} & \textbf{98.2} & \betterinv{0.1} \\
\end{tabular}
\caption{\textbf{Results on smaller classification datasets.} While the standard SVRG mostly hurts the performance, \approach\ decreases the training loss and increases the validation accuracy.}
\label{tab:pre-trained2}
\end{table}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/tables/recipe.tex <==
\begin{table}[h]
\centering
\small
\addtolength{\tabcolsep}{-.3pt}
\def\arraystretch{1.2}
\begin{tabular}{y{146}|x{98}}
config & value \\
\Xhline{0.7pt}
weight init  & trunc. normal (0.2) \\
optimizer & AdamW \\
base learning rate & 4e-3 \\
weight decay & 0.05 \\
optimizer momentum & $\beta_1, \beta_2=0.9, 0.999$ \\
learning rate schedule & cosine decay \\
warmup schedule & linear \\
randaugment \citep{randaugment} & (9, 0.5) \\
mixup \citep{zhang2018mixup} & 0.8 \\
cutmix \citep{yun2019cutmix} & 1.0 \\
random erasing \citep{randomerasing} & 0.25 \\
label smoothing \citep{label-smoothing} & 0.1
\end{tabular}
\caption{\textbf{Our basic training recipe,} adapted from ConvNeXt \citep{convnextzhuang}.}
\label{tab:recipe}
\end{table}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/tables/schedule.tex <==
\begin{table}[h]
\def\arraystretch{1.3}
\centering
\small
\begin{tabular}{lcccccc}
train loss & linear & quadratic & geometric & d-linear & d-quadratic & d-geometric \\
\Xhline{0.7pt}
\( \alpha_0=0.5\) & \textbf{1.59}	& 1.61	& 1.62	& 2.07	& 1.97	& 1.81\\
\( \alpha_0=0.75\) & \textbf{1.57} & 1.58 & 1.58 & 2.07 & 2.00 & 1.93\\
\( \alpha_0=1\) & 1.57 &	\textbf{1.56} &	1.57 &	2.00 &	1.97 & 1.88\\
\end{tabular}
\caption{\textbf{Schedules.} \textbf{Bold} indicates the lowest training loss among different schedules using the same initial coefficient (row). \approach\ with global schedules outperforms that with double schedules.}
\label{tab:schedule}
\end{table}


==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/tables/seed.tex <==
\begin{table}[h]
\centering
\small
\def\arraystretch{1.3}
\addtolength{\tabcolsep}{5pt}
\begin{tabular}{lcccccccc}
& \multicolumn{2}{c}{CIFAR-100} & \multicolumn{2}{c}{Pets} & \multicolumn{2}{c}{Flowers} & \multicolumn{2}{c}{STL-10} \\
\Xhline{0.7pt}
AdamW & \multicolumn{2}{c}{2.645\ \(\pm\)\ 0.013} & \multicolumn{2}{c}{2.326\ \(\pm\)\ 0.088} & \multicolumn{2}{c}{2.436\ \(\pm\)\ 0.038} & \multicolumn{2}{c}{1.660\ \(\pm\)\ 0.017} \\
\rowcolor{gray}
+\ \approach\ & \multicolumn{2}{c}{\textbf{2.606}\ \(\pm\)\ 0.017} & \multicolumn{2}{c}{\textbf{2.060}\ \(\pm\)\ 0.071} & \multicolumn{2}{c}{\textbf{2.221}\ \(\pm\)\ 0.042} & \multicolumn{2}{c}{\textbf{1.577}\ \(\pm\)\ 0.022}\\
\end{tabular}

\centering
\small
\begin{tabular}{lcccccccc}
& \multicolumn{2}{c}{Food-101} & \multicolumn{2}{c}{DTD} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{EuroSAT} \\
\Xhline{0.7pt}
AdamW & \multicolumn{2}{c}{2.478\ \(\pm\)\ 0.021} & \multicolumn{2}{c}{2.072\ \(\pm\)\ 0.066} & \multicolumn{2}{c}{1.583\ \(\pm\)\ 0.005} & \multicolumn{2}{c}{1.259\ \(\pm\)\ 0.017}\\
\rowcolor{gray}
+\ \approach\ & \multicolumn{2}{c}{\textbf{2.426}\ \(\pm\)\ 0.007} & \multicolumn{2}{c}{\textbf{1.896}\ \(\pm\)\ 0.075} & \multicolumn{2}{c}{\textbf{1.572}\ \(\pm\)\ 0.011} & \multicolumn{2}{c}{\textbf{1.239}\ \(\pm\)\ 0.016}\\
\end{tabular}
\caption*{(a) \textbf{training loss}}
\vspace*{0.2cm}

\begin{tabular}{lcccccccc}
& \multicolumn{2}{c}{CIFAR-100} & \multicolumn{2}{c}{Pets} & \multicolumn{2}{c}{Flowers} & \multicolumn{2}{c}{STL-10} \\
\Xhline{0.7pt}
AdamW & \multicolumn{2}{c}{81.02\ \(\pm\)\ 0.07} & \multicolumn{2}{c}{70.61\ \(\pm\)\ 1.55} & \multicolumn{2}{c}{80.33\ \(\pm\)\ 1.01} & \multicolumn{2}{c}{80.80\ \(\pm\)\ 1.46} \\
\rowcolor{gray}
+\ \approach\ & \multicolumn{2}{c}{\textbf{81.07}\ \(\pm\)\ 0.22} & \multicolumn{2}{c}{\textbf{76.37}\ \(\pm\)\ 1.06} & \multicolumn{2}{c}{\textbf{84.15}\ \(\pm\)\ 1.15} & \multicolumn{2}{c}{\textbf{83.65}\ \(\pm\)\ 0.92} \\
\end{tabular}

\centering
\small
\begin{tabular}{lcccccccccc}
& \multicolumn{2}{c}{Food-101} & \multicolumn{2}{c}{DTD} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{EuroSAT} \\
\Xhline{0.7pt}
AdamW & \multicolumn{2}{c}{85.29\ \(\pm\)\ 0.47} & \multicolumn{2}{c}{56.21\ \(\pm\)\ 1.19} & \multicolumn{2}{c}{94.29\ \(\pm\)\ 0.67} & \multicolumn{2}{c}{97.91\ \(\pm\)\ 0.12} \\
\rowcolor{gray}
+\ \approach\ & \multicolumn{2}{c}{\textbf{85.45}\ \(\pm\)\ 0.43} & \multicolumn{2}{c}{\textbf{61.44}\ \(\pm\)\ 0.35} & \multicolumn{2}{c}{\textbf{94.94}\ \(\pm\)\ 0.60} & \multicolumn{2}{c}{\textbf{98.13}\ \(\pm\)\ 0.07}
\end{tabular}
\caption*{(b) \textbf{validation accuracy}}
\caption{\textbf{Results of {$\boldsymbol{\alpha}$-SVRG} with AdamW with standard deviation.}}
\label{tab:seed}
\end{table}

==> jjynsjddzmtfzjvwczmvkvsbmwsdptsx/tables/seed_2.tex <==
\begin{table}[th]
\centering
\small
\def\arraystretch{1.3}
\addtolength{\tabcolsep}{5pt}
\begin{tabular}{lcccccccc}
	
& \multicolumn{2}{c}{CIFAR-100} & \multicolumn{2}{c}{Pets} & \multicolumn{2}{c}{Flowers} & \multicolumn{2}{c}{STL-10} \\
\Xhline{0.7pt}
SGD & \multicolumn{2}{c}{3.118\ \(\pm\)\ 0.035} & \multicolumn{2}{c}{2.706\ \(\pm\)\ 0.095} & \multicolumn{2}{c}{2.822\ \(\pm\)\ 0.058} & \multicolumn{2}{c}{1.763\ \(\pm\)\ 0.032} \\
\rowcolor{gray}
+\ \approach\ & \multicolumn{2}{c}{\textbf{3.087}\ \(\pm\)\ 0.011} & \multicolumn{2}{c}{\textbf{2.655}\ \(\pm\)\ 0.134} & \multicolumn{2}{c}{\textbf{2.699}\ \(\pm\)\ 	0.049} & \multicolumn{2}{c}{\textbf{1.725}\ \(\pm\)\ 0.043}\\
\end{tabular}
	
\centering
\small
\begin{tabular}{lcccccccc}
& \multicolumn{2}{c}{Food-101} & \multicolumn{2}{c}{DTD} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{EuroSAT} \\
\Xhline{0.7pt}
SGD & \multicolumn{2}{c}{3.424\ \(\pm\)\ 0.015} & \multicolumn{2}{c}{2.589\ \(\pm\)\ 0.032} & \multicolumn{2}{c}{1.789\ \(\pm\)\ 0.029} & \multicolumn{2}{c}{1.449\ \(\pm\)\ 0.029}\\
\rowcolor{gray}
+\ \approach\ & \multicolumn{2}{c}{\textbf{3.397}\ \(\pm\)\ 0.006} & \multicolumn{2}{c}{\textbf{2.543}\ \(\pm\)\ 0.039} & \multicolumn{2}{c}{\textbf{1.764}\ \(\pm\)\ 0.014} & \multicolumn{2}{c}{\textbf{1.412}\ \(\pm\)\ 0.011}\\
\end{tabular}
\caption*{(a) \textbf{training loss}}
\vspace*{0.2cm}









	
	
	


\begin{tabular}{lcccccccc}
& \multicolumn{2}{c}{CIFAR-100} & \multicolumn{2}{c}{Pets} & \multicolumn{2}{c}{Flowers} & \multicolumn{2}{c}{STL-10} \\
\Xhline{0.7pt}
SGD & \multicolumn{2}{c}{75.43\ \(\pm\)\ 0.88} & \multicolumn{2}{c}{71.25\ \(\pm\)\ 4.74} & \multicolumn{2}{c}{65.92\ \(\pm\)\ 4.24} & \multicolumn{2}{c}{76.09\ \(\pm\)\ 1.09} \\
\rowcolor{gray}
+\ \approach\ & \multicolumn{2}{c}{\textbf{75.93}\ \(\pm\)\ 0.83} & \multicolumn{2}{c}{\textbf{71.89}\ \(\pm\)\ 4.84} & \multicolumn{2}{c}{\textbf{74.98}\ \(\pm\)\ 3.14} & \multicolumn{2}{c}{\textbf{78.55}\ \(\pm\)\ 2.54} \\
\end{tabular}

\centering
\small
\begin{tabular}{lcccccccccc}
& \multicolumn{2}{c}{Food-101} & \multicolumn{2}{c}{DTD} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{EuroSAT} \\
\Xhline{0.7pt}
SGD & \multicolumn{2}{c}{60.58\ \(\pm\)\ 2.00} & \multicolumn{2}{c}{57.53\ \(\pm\)\ 1.25} & \multicolumn{2}{c}{91.10\ \(\pm\)\ 1.31} & \multicolumn{2}{c}{
95.31\ \(\pm\)\ 0.46} \\
\rowcolor{gray}

+\ \approach\ & \multicolumn{2}{c}{\textbf{62.89}\ \(\pm\)\ 0.87} & \multicolumn{2}{c}{\textbf{58.44}\ \(\pm\)\ 1.05} & \multicolumn{2}{c}{\textbf{91.60}\ \(\pm\)\ 0.59} & \multicolumn{2}{c}{\textbf{96.17}\ \(\pm\)\ 0.17}
\end{tabular}
\caption*{(b) \textbf{validation accuracy}}
\caption{\textbf{Results of {$\boldsymbol{\alpha}$-SVRG} with SGD on smaller datasets with standard deviation.}}
\label{tab:seed_2}
\end{table}
